On Technical Trading and Social Media Indicators in Cryptocurrencies' Price Classification Through Deep Learning

This work aims to analyse the predictability of price movements of cryptocurrencies on both hourly and daily data observed from January 2017 to January 2021, using deep learning algorithms. For our experiments, we used three sets of features: technical, trading and social media indicators, considering a restricted model of only technical indicators and an unrestricted model with technical, trading and social media indicators. We verified whether the consideration of trading and social media indicators, along with the classic technical variables (such as price's returns), leads to a significative improvement in the prediction of cryptocurrencies price's changes. We conducted the study on the two highest cryptocurrencies in volume and value (at the time of the study): Bitcoin and Ethereum. We implemented four different machine learning algorithms typically used in time-series classification problems: Multi Layers Perceptron (MLP), Convolutional Neural Network (CNN), Long Short Term Memory (LSTM) neural network and Attention Long Short Term Memory (ALSTM). We devised the experiments using the advanced bootstrap technique to consider the variance problem on test samples, which allowed us to evaluate a more reliable estimate of the model's performance. Furthermore, the Grid Search technique was used to find the best hyperparameters values for each implemented algorithm. The study shows that, based on the hourly frequency results, the unrestricted model outperforms the restricted one. The addition of the trading indicators to the classic technical indicators improves the accuracy of Bitcoin and Ethereum price's changes prediction, with an increase of accuracy from a range of 51-55% for the restricted model, to 67-84% for the unrestricted model.

==> related_works.tex <==
\section{Related Works}
\label{sec:relatedworks}


Cryptocurrencies have seen recent demand and price spikes. 
It has been discovered that cryptocurrency prices and some online and social media variables tend to be linked to time intervals. 
Moreover, it has been reported that cryptocurrencies are vulnerable to bubble-like price growth intervals. 
The theory investigated how factors such as price and online variables depend on the consumer regime.

The fluctuating properties of the rapidly evolving Bitcoin market are measured over selected sub-periods, in terms of return distributions, volatility autocorrelation, Hurst exponents, and multiscaling effects, based on 1-min price changes reported since 2012 \cite{matta2015bitcoin}.
These fluctuations have been studied in correlation to the phenomena of Initial Coin Offer (ICO) which gave a boost to the cryptocurrencies markets ecosystem \cite{hartmann2018evaluation, hartmann2019alternative}.

Although high-frequency pricing data has been available since the start of trading, Bitcoin provides a rare insight into the statistical features of the trajectory of market maturation. 
The advent of money has been one of the most important accomplishments of civilizations in history, which conditions their further development at the same time.

Quantitative investigations aimed at extracting information from cryptocurrencies prices time series and predicting prices drivers \cite{phillips2018cryptocurrency, bartolucci2020butterfly} or the next most likely jump, spanning from theoretical models of pricing and adoption of digital tokens \cite{econBTC,econBTC2,SBAK} to machine learning \cite{baroprediction, returnsprediction} and neural network-driven \cite{NNprediction} forecasts of prices and returns. Other investigations look at relationships among cryptocurrencies' development communities and price changes \cite{bartolucci2020butterfly, destefanis2017randomness} and the social factors which drives  cryptocurrencies' development communities \cite{destefanis2018measuring, ortu2018mining, murgia2012refactoring}.


Analysis of the cryptocurrency markets \cite{drozdz1,drozdz2,scirepclustering,urquhart2016} have yielded insights on their maturity, efficiency and structure. A large body of literature is also looking at the volatility of cryptocurrencies, from the model estimation point of view \cite{katsiampa2017volatility,lahmiri2018long} as well as by extrapolating the mechanisms driving the fluctuations: several studies showed for example  a strong correlation with global economic activity \cite{volatilityconrad, walther} and volume of trades \cite{bouri2019trading,chen2020bitcoin,mcnally2018predicting}.
